Multi-Modal End-User Programming of Web-Based Virtual Assistant Skills

While Alexa can perform over 100,000 skills on paper, its capability covers only a fraction of what is possible on the web. To reach the full potential of an assistant, it is desirable that individuals can create skills to automate their personal web browsing routines. Many seemingly simple routines, however, such as monitoring COVID-19 stats for their hometown, detecting changes in their child's grades online, or sending personally-addressed messages to a group, cannot be automated without conventional programming concepts such as conditional and iterative evaluation. This paper presents VASH (Voice Assistant Scripting Helper), a new system that empowers users to create useful web-based virtual assistant skills without learning a formal programming language. With VASH, the user demonstrates their task of interest in the browser and issues a few voice commands, such as naming the skills and adding conditions on the action. VASH turns these multi-modal specifications into skills that can be invoked invoice on a virtual assistant. These skills are represented in a formal programming language we designed called WebTalk, which supports parameterization, function invocation, conditionals, and iterative execution. VASH is a fully working prototype that works on the Chrome browser on real-world websites. Our user study shows that users have many web routines they wish to automate, 81% of which can be expressed using VASH. We found that VASH Is easy to learn, and that a majority of the users in our study want to use our system.

==> design.tex <==

\section{Design and Rationale}
\VASH and \WebTalk were designed hand-in-hand. It is a balancing act to make the specification intuitive to the user, while giving them the power of programming.  For example, we have made it possible for users to define many functions without learning about variables.  
Here we provide a high-level overview of the challenges and design choices:
\begin{itemize}
\item 
\textit{\Webops}. We need to record and replay actions, in a manner that is robust to changes in the content of the page. We use CSS selector, as a way to address elements on the page that depends only on the semantic structure and not the actual content.
\item
\textit{Selection}. The native browser selection allows the user to easily refer to a single element in the page. Native selection is not sufficient when the user wants to select multiple elements (such as a list or table column), especially with complex page layouts, so we also introduce an explicit selection mode.
\item
\textit{Function definitions with parameters}. To automate actions on the web, we need to define and invoke functions, and we need to parameterize them. We leverage the familiar copy and paste as a way to describe parameters and variables implicitly, which keeps the simple cases simple. To support more advanced cases, we also introduce named parameters and named variables.
\item
\textit{Conditionals}. We need to capture conditions explicitly, which are not shown in the demonstration. Condition is type based, and it can be applied to a single action or a function call. There is no else clause because PBD needs to work with concrete values exhibiting the condition of interest. 
\item
\textit{Iteration}. To avoid the complexity of while loops, iteration occurs over a list of selected elements. Similarly, there is also no recursion. This is a trade-off in computation power vs. simplicity.
\item
\textit{Aggregation}. We wish to compute results that are not visible on the page, in particular aggregation operations (min, max, sum, etc.) over multiple selected elements. This is necessary when the user is computing the result in their mind (to replay at a later time), and useful when computing by hand is too tedious.
\item
\textit{On-demand function definition}. The user might not realize they need a helper function until half-way through recording their main function. Unlike coding in an IDE, there is no jumping around in a file to add it somewhere else. Instead, function specification can be nested freely, so they can be defined at the point of use.
\end{itemize}

\iffalse
\subsection{\Webops}

\iffalse
\begin{lstlisting}
@load(url="https://finance.yahoo.com");
@set_input(selector="input#search", text="goog");
@click(selector="button[type=submit]");
let this := @select(selector="span#today-quote");
\end{lstlisting}
\fi


With \VASH, every action the user normally takes on the web is captured as a \WebTalk web primitive, which can be executed to get the same effect as the user's action. An example of the actions captured while recording the stock skill is shown in Table~\ref{table:basic_example} (lines 2 to 4).

The requirement is to execute exactly the same operations that the user demonstrates. First, the webpage opened at the time of the recording is explicitly loaded in the WebTalk program. Furthermore, all actions that invoke responses from the website must be remembered and replayed. We record all navigations between pages, keyboard input in forms, mouse clicks on buttons, links, tabs in the browser, as well as copy and paste. The corresponding \WebTalk \webops are shown in the table.

We do not need to record operations such as scrolling or changing keyboard or mouse focus, as those operations only affect the view of the users. Drawing with the mouse, which involves a click and a drag, is not currently supported.

\paragraph{CSS Selectors for Specifying Targets}
To execute the same operation that the user demonstrates, all demonstrated actions have to be uniquely identified on the page: which button was clicked, where text was entered, which tables were selected. Additionally, to support replaying the action at a later time, the identification of the element cannot depend on the absolute position of the specific element, or the content of the element, because those attributes would change when the page changes.

\VASH uses CSS (Cascading Style Sheets) selectors~\cite{cssselectors}, a language for describing a subset of HTML elements in a page, originally designed for styling. CSS selectors use semantic information to identify the elements (HTML tag name, author-specified ID and class on each element), positional and structural information (ordinal position in document order, parent-child relationship), and content information.

When recording the action, \VASH records which elements the user is interacting with, and generates a CSS selector that identifies that element uniquely. When available, \VASH uses ID and class information to construct the selector, falling back to positional selectors when those information are not sufficient to uniquely identify the element. As such, the CSS selectors employed by \VASH are robust to changes in the content of the page and small changes in layout. This means that \VASH selectors work best with static HTML pages where IDs and classes are assigned according to the semantic meaning of each element. Conversely, \VASH cannot work with fully randomly generated CSS classes (such as those used by the popular React library). We note that previous work has suggested using computer vision to generate more semantic selectors for elements~\cite{Sereshkeh_2020}, so this restriction could be lifted in the future.
% For each element that the user interacts  A unique selector of the DOM element on any page is generated for each action that is then fed into \VASH.
\iffalse
The Finder \cite{finder} library is used to generate the 
\fi

\paragraph{Select, copy and paste}

\VASH records all select, copy and paste operations. The copy operation is converted to a ``select'' web primitive (Table~\ref{table:webops}), which refers to the element that were selected when the copy was executed, rather than recording the specific value copied. 

If both the copy and paste are executed in the browser in the same recording session, the paste operation is converted to a ``set input'' web primitive that refers to the result of the select web primitive (Table~\ref{table:webops}). 
Suppose a user copies a stock symbol from a webpage, which happens to be embedded in a HTML element with ID ``stock'', which is then pasted in a HTML ``input'' element with ID ``search'', then the following \WebTalk code is generated:

\small
\begin{tabbing}
12345\=12345\=\kill
\>$\textbf{let}~\text{this} := @\text{select}(\textit{selector}=\text{``\#stock''});$\\
\>$\text{this} \Rightarrow @\text{set\_input}(\textit{selector}=\text{``input\#search''}, \textit{value}=\text{this}.\text{text});$
\end{tabbing}
\normalsize

In this code, the result of the ``select'' web primitive is bound to the special ``this'' variable, which is then used in the subsequent ``set input'' web op. ``this'' is a special variable that is implicitly defined and accessed while recording web operations. It is a table of HTML elements, and it records the \textit{text} content and the \textit{number} value.
When this \WebTalk code is replayed, the text of the "\#stock" element is selected, and set as the value of "input\#search" element, as if the user was copy-pasting.

On the other hand, if the copy operation is not recorded in the browser (i.e. the data copied comes from another app), the paste operation is recorded as ``type'' web primitive, containing the constant value being pasted, as if the user typed it explicitly (Table~\ref{table:webops}).

\iffalse
Cut operations are recorded similarly to copy operations, but \VASH also erases the content of the element the user cut from, if the element is editable.
\fi

\subsection{Functions}
\subsubsection{Basic function definition and invocation}
Here we first introduce the basic components of function definition and invocation. 
A function is defined by wrapping a ``start recording <func-name>'' command and a ``stop recording'' command around the function body (Table~\ref{table:constructs}). Upon hearing the ``stop recording'' command. At that point, the sequence of recorded \WebTalk web operations is wrapped in a \WebTalk function definition, with the name provided by the user.

While recording the function, the user can issue the command ``return this'', which returns what is currently selected (Table~\ref{table:constructs})
\iffalse
In \WebTalk, this is expressed as:
\begin{lstlisting}
let this := @select(select="#quote");
this => notify;
\end{lstlisting}
\fi
At most one return statement can appear in the function, but the return statement need not be last: it can be followed by additional web ops, which do not affect the return value. This allows the function to perform ``clean up'' actions (such as logging out) before returning the result.

\VASH creates an implicit parameter when it records a paste operation that originates from a copy outside the function. The paste web primitive generates a ``set input'' web operation modified to use the formal parameter (Table~\ref{table:complex_example}, line~\ref{exampleline:complex_example:set_input_1}). An example of a function with an implicit parameter is shown in Table~\ref{table:basic_example}.

Users can also create explicitly named parameters, by saying ``this is BLA'' while an input element is selected (Table~\ref{table:constructs}).
This allows a function to have multiple parameters.

Once the function is defined, the user can ask their assistant to execute it. The user can say ``call <func-name>'' to call a function without parameters. They can call a function with parameter by saying
``call <func-name> with this'', in which case the actual parameter is set to the result of the current selection (Table~\ref{table:basic_example}, line 10). If the function returns a result, the result is assigned to the ``this'' variable (Table~\ref{table:complex_example}, line~\ref{exampleline:complex_example:set_this_result}).

\subsubsection{Function Invocations in Functions}
Functions may also be called inside functions. In a PBD system where the user is always dealing with concrete values, we need to execute the function called, so the result can be returned to allow the user continue with the demonstration.  If the called function returns a result, the result is displayed as a popup on top of the current page.

Furthermore \VASH lets users define another function inside a function, because the user would not know what helper functions are needed ahead of time, and the user would not have the context to use PBD to define the function. For simplicity, all functions have global scope, meaning that they can be invoked anywhere, and they cannot use any variables from the lexical scope of the function definition.

Imagine that Bob wants to invite friends over for dinner, but he wants to pick a recipe that does not cost more than \$30. He creates a skill that looks up a recipe on allrecipes.com and uses Walmart.com to find the cost of each of the ingredients, and sums it up, as shown in Table~\ref{table:complex_example}. He visits the ``World's Best Lasagna'' page and sees that there is a long list of ingredients. He does not want to do it one by one, so he realizes that he needs to create a helper function for the price. As shown in this example, Bob defines the ``price'' function inside the ``recipe'' function; and invokes the ``price'' function on all the ingredients. The result of the ``price'' function is shown to the user and saved to the current selection. Bob sees all the Walmart prices on the ingredients of this recipe, he then asks \VASH to compute the sum of all the ingredients, returns the result, and finishes defining the ``recipe'' function. He can now apply this function to any other recipes by invoking ``recipe'' on them.

\subsection{Control Constructs}
Recorded web operations and functions can be combined with control constructs to describe more complex computation. These control constructs are introduced with voice commands while the user is recording the function.

\iffalse
\paragraph{Conditional}
\TODO{GC: This description of the conditional does not match the Construct Table. The table has conditional only on function calls (which is both what we need, and what we implemented), while this paragraph has general conditionals. I'm tempted to kill general conditionals.}
If the user's action is dependent on the data displayed, the user will describe the logic to the system, so it is encoded in \WebTalk and replayed when the function is invoked later. The user introduces the conditional by issuing the command ``do the following if <condition>''. The next function invocation command or web primitive is then made conditional on the provided condition. For example, if the user says ``do the following if this is greater than 100'' and then clicks a button, \VASH generates the following \WebTalk:

\begin{tabbing}
123\=\kill
\>$\text{this}, \textit{number} > 100 \Rightarrow @\text{click}(\textit{selector}=\ldots);$\\
\end{tabbing}

% For example, the user picks a restaurant because it has the highest rating, the user simply needs to articulate that to the system.  

The filter is only applied to the command or web op immediately following the condition. Conditional return commands either return the result, or return nothing: the control flow of the function is not affected. This is because, in a PBD system, only data flow can be recorded, not control flow.
 As a shortcut, the user can also issue commands of the form ``call <func-name> if <condition>'' and ``return this if <condition>'', which combines the condition command with another voice command.

Our current system only supports a single predicate, which can use equality, inequality, or comparison between the current selection and a constant. As the natural language technology improves, we expect in the future to support arbitrary logical operations (and, or, not). 
\fi

\iffalse
\begin{figure*}
\small

\begin{verbatim}
VOICE OPERATIONS               GUI OPERATIONS                                PROGRAM
Start Get Rest. on "Italian"   Select "Italian" on the Webber dialogue       Get_Restaurants (param) {
                               Type Yelp.com.                                  @Load (Yelp.com)
                               <PASTE> and type "Manhattan" into Yelp.com.     @Paste <SELECTED> and type "Manhattan" into Yelp.com
                               Enter
Start Get location on this     Select first restaurant.                      Get_location (param) { // a top level function
                               Click first restaurant                          @Click param - load url
If this is > 4                 Select number-of-stars                          If <SELECTED> is greater than 4
Return this                    Select location                                    return <SELECTED> 
Stop Get location                                                            }
                               Select the list of restaurants
                               Call Get location on the first 5 items          Get_location [on 5 items] <SELECTED> 
Return this                    Select result in the Webber dialogue            Return <SELECTED>	
Stop Get Restaurant                                                         }
\end{verbatim}

\caption{Full Example}
\label{fig:full_example}
\end{figure*}
\fi

\iffalse
\subsection{Scoping}

Depth-first specification.
Meta-commands to Webber: these commands can be nested in the definition of another function, but proper nesting is checked. 
\fi

\paragraph{Iteration}
If a function is invoked by passing the current selection (``call <func-name> with this''), it is applied to each element in the selection individually. If the selection consists of a list of elements, the function iterates over the list (Table~\ref{table:constructs}, line 4).

Iteration can also be made conditional, by adding a predicate (Table~\ref{table:constructs}, line 3). In this case, the function is only applied to the list elements that satisfy the predicate. For example, ``call func with this if this is greater than 100'' can be expressed as:
\begin{tabbing}
123\=\kill
\>$\text{this}, \textit{number} > 100 \Rightarrow \text{func}(\textit{p\_this}=\text{this}.\text{text});$
\end{tabbing}

\textit{number} is a field of the currently selected HTML elements (in the ``this'' variable) and it is computed by extracting any numeric value in the elements. Our current system only supports a single predicate, which can use equality, inequality, or comparison between the current selection and a constant. As the natural language technology improves, we expect in the future to support arbitrary logical operations (and, or, not). 

\paragraph{Aggregation}
\WebTalk supports all the aggregation operations supported by ThingTalk with database extensions~\cite{xu2020schema2qa}.  Once a set of numbers is selected in either a table or list, the \textit{sum},  \textit{count}, \textit{average}, \textit{max}, and \textit{min} can be computed and returned, by issuing the voice command ``calculate the <operation> on this''. For example, the sum of all selected elements can be computed by saying ``calculate the sum of this'' (Table~\ref{table:complex_example}, line~\ref{exampleline:complex_example:calculate_sum}).
\iffalse
which generates the following \WebTalk:
\begin{tabbing}
123\=\kill
\>$\textbf{let}~\textit{sum} := \textbf{aggregate}~\text{sum}~ \textit{number}~\textbf{of}~\text{this};$\\
\end{tabbing}
\fi

The result of the aggregation is immediately displayed to the user. After computing the aggregation, the user can issue the command ``return the sum'' (respectively ``the count'', ``the average'', etc.), to use the aggregation result as the result of the current function (Table~\ref{table:complex_example}, line~\ref{exampleline:complex_example:return_sum}), or they can use the ``sum'' in a subsequent conditional command.

\paragraph{Named Variables}
In addition to the ``this'' variable that is implicitly manipulated by selection and copy-paste operation, users can optionally create explicit named variables. This allows the user to manipulate multiple selections at once; this is in particular useful when combined with conditionals. Named variables are created by selecting some elements on the page, and issuing the control command ``this is a <var-name>'' (Table~\ref{table:constructs}). 
Named variables can be used in place of ``this'' in conditional, function invocation and return statements.
\iffalse
For example, in the stock case, the user can select the current quote, and say ``this is a quote'', and they can select the daily increase, and say ``this is the increase''. This generates the following \WebTalk code:

\begin{lstlisting}
let quote := @select(select="#quote");
let increase := @select(select="#increase");
\end{lstlisting}
. For example, the user can issue the command ``return the quote if the increase is greater than 10'', in which case the following \WebTalk is generated:
% handwaving the syntax here a little bit...
\begin{lstlisting}
quote, increase >= 10 => notify;
\end{lstlisting}
\fi

\iffalse
\subsubsection{Start Selection}
Variables and data are selected by the user so that they can be later named.  A user specifies that they are beginning and the plugin changes modes to override the native selection of the browser.  The new selection is able to select columns of tables, rows of tables, individual numbers, text, and list elements. 

Example paraphrases: 
``begin selection'',
% ``start selection'',
% ``start select''

\subsubsection{Stop Selection}
When the user has selected all the data that want to be named, they tell the system to go back to the native selection process.

Example paraphrases: 
``stop selection'',
% ``stop select'',
% ``end selection''


\subsubsection{Variables}
\subsubsection{Name variable}

Variables need to be named for them to work with the program.  Once a variable is named on the page it is remembered so that it can be used later.  In addition, the variable is shown with a highlight over the text so that the user is able to recall which variable they named what.

The selection starts by having the user select the data that is ended by the program.  They do so by doing a dragging motion over the top of the data.  A box appears on top.  The computer then prompts the user to say the name of the data that they are creating.

The selected data is then processed by the system to determine if it is a single element or a list of elements.  This is done by looking at the accompanying HTML to determine if it is  a div or table.  Once the data is selected and named it can be used as a parameter for a skill.

Variables are named on a page to be used as input to programs.  Once a variable is named it can be used in any program.  To name a variable, a user first select is using the selection mechanism.  

% If the user wants a constants value.  Things that are relative values.

Example paraphrases: 
``this is a \texttt{*var\_name}''
% ``this is an \texttt{*var\_name}'',
% ``these are \texttt{*var\_name}'',
% ``this variable is a \texttt{*var\_name}''

\subsection{Alternative execution paths}
Limitation and future work.

\subsubsection{Run Program}
There are multiple ways to run a program depending on the number of parameters that are required by the program.  If no variables are required the user only says the name of the program to run.

Example paraphrases: 
``call \texttt{:prog\_name}'',
% ``run \texttt{:prog\_name}''

\subsubsection{Run Program With Parameters}
Some programs require parameters to be specified.

If just one or two parameters is needed,  
Example paraphrases: 
``call \texttt{:prog\_name} with \texttt{:var\_name}'',
% ``call \texttt{:prog\_name} using \texttt{:var\_name}'',
% ``run \texttt{:prog\_name} with \texttt{:var\_name}'',
% ``run \texttt{:prog\_name} using \texttt{:var\_name}''.

Web Automator can run programs with up to two parameters.

Example paraphrases: 
``call \texttt{:prog\_name} using \texttt{:var\_name\_1} and \texttt{:var\_name\_2}'',
% ``call \texttt{:prog\_name} with \texttt{:var\_name\_1} and \texttt{:var\_name\_2}'',
% ``run \texttt{:prog\_name} using \texttt{:var\_name\_1} and \texttt{:var\_name\_2}'',
% ``run \texttt{:prog\_name} with \texttt{:var\_name\_1} and \texttt{:var\_name\_2}'',

\subsubsection{Run program with scheduling}
Programs can be scheduled to run at a later time.   

Example paraphrases: 
``run \texttt{:prog\_name} at \texttt{*time'}'',
% ``run \texttt{:prog\_name} with \texttt{:var\_name} at \texttt{*time}''


\subsubsection{Run program from another Program}
Programs can be called and created within other programs.

Example paraphrases: 
``run \texttt{:prog\_name} at \texttt{*time'}'',
% ``run \texttt{:prog\_name} with \texttt{:var\_name} at \texttt{*time}''



\begin{comment}
\subsubsection{Copy and paste}
Copy and paste is feature that many users are familiar with and use everyday.  It allows people to pipe data from one context to another, thereby connecting otherwise unlike programs.  In a programming by demonstration environment, where multiple types of applications need to be connected, this functionality is essential.

\subsubsection{Mouse Clicks}
A powerful means of programming by demonstration is the mouse click.  User can click on links, button, menu within the browser page.  Click are also recorded in the browser also.  A user can click on a tab in the browser and the system will record that the tab has been switched and it will be part of the program.

\subsubsection{Typing}
When filling out a form or typing an email, users need to be able to type text that they want the system to automate.  Once the system is in record mode, keystrokes are recorded and placed in the point that CSS selector.


\subsubsection{Starting a Function}
% \subsection{Start recording}
To begin a session the user has to specify when the browser plugin should start recording the actions of the user.
When the user starts recording actions clicks, keystrokes, and browser navigations are logged.
In the upper right hand corner of the browser a red light appears to let the user know that their actions are being recorded.

% Paraphrases:
% ``start recording''.

The program has to be named so that it can be called later by the user.  One a program is named it is added to the database of programs and can be invoked later or shared.  Once saved, the user can see all of their programs in a ``App Store'' where they can also review the underlying ThingTalk code that was generated.

If a user finds that they need to build another program while already recording another program, they can start recording a new program while a current program is already recording.  By allowing for nested recordings to take place, we enable XXX.  



Example Paraphrases: 
``start a function called  \texttt{:program\_name}'',
% ``call this command \texttt{:var\_name}'',
% ``name this command \texttt{:var\_name}'',
% ``name this program \texttt{:var\_name}'',
% ``this program is \texttt{:var\_name}'',
% ``this program is called \texttt{:var\_name}'',
% ``this program should be called \texttt{:var\_name}''

\subsubsection{Stop recording}
When the user has completed their program, they tell the computer that it should no longer log the events for the most recent function.

Example paraphrases: 
``stop function''

To Almond
Get stocks.                                                     Get\_Stocks(); 
Get stocks at 8am every day.                                    @8am => get stocks () => notify 

\end{comment}
\fi

\iffalse
In the stock example, \VASH generates:

\begin{lstlisting}
function get_stocks() {
  @load(url="https://finances.yahoo.com");
  @set_input(selector="input#search", text="goog");
  @click(selector="button[type=submit]");
}
\end{lstlisting}
\fi

\iffalse
Functions can be called via the Assistant or inside a function, with the user command ``run <func-name>'' (Table~\ref{table:constructs}). For example, the user can issue the ``stocks'' function with the command ``run stocks''.

In \WebTalk, this is written:
\begin{lstlisting}
get_stocks();
\end{lstlisting}
To support programming by demonstration, where functions are not defined ahead of time, \VASH allows users to nest function declarations, that is, in the middle of recording a function, the user can start recording another function.  All functions defined have a global scope to keep the programming model simple. 
\fi

\iffalse
For example, if the user pastes in the input box while recording the ``stocks'' example, \VASH would generate the following \WebTalk code:

\begin{lstlisting}
function get_stocks(p_this : String) {
  @load(url="https://finances.yahoo.com");
  @set_input(selector="input#search", text=this);
  @click(selector="button[type=submit]");
}
\end{lstlisting}
\fi

\iffalse
At a later time, to invoke the function, the user can say "call get stocks with IBM", in which case the actual parameter is bound to the constant IBM:
\begin{lstlisting}
get_stocks(p_this="IBM");
\end{lstlisting}
\fi

\iffalse
\begin{tabbing}
12\=3456\=\kill
$\textbf{let}~\text{this} := @\text{select}(\textit{selector}=\ldots);$\\
$\text{this} \Rightarrow \text{stocks}(\textit{p\_this}=\text{this}.\textit{text});$
\end{tabbing}
\fi


\iffalse
For example, an email procedure can be written as:
\begin{lstlisting}
function send_email(p_address : String,
                    p_subject : String) {
  @load(url="https://mail.google.com");
  @set_input(selector="#to", text=p_address);
  @set_input(selector="#subject", text=p_subject);
  @set_input(selector="#body", text="...");
  @click(selector="button[type=submit]");
}
\end{lstlisting}
\fi

\iffalse
For example, while recording the stock example, the user can select the search box, and say ``this is a symbol'', to generate:

\begin{lstlisting}
function get_stocks(p_symbol : String) {
  @load(url="https://finances.yahoo.com");
  @set_input(selector="input#search", text=p_symbol);
  @click(selector="button[type=submit]");
}
\end{lstlisting}
 
When recording this procedure, the user will say ``this is a recipient'' while entering the ``To'' field, and ``this is a subject'' in the ``Subject'' field (Table~\ref{table:constructs}).

Functions with named parameters are invoked by naming the parameters explicitly, for example ``call get stocks with symbol IBM'', or ``call send email with recipient bob@example.com and subject hello''.
\fi
\fi

==> design_principles.tex <==
%NO LONGER IN USE
\section{Design Principles}

\subsection{Everything is a Variable}

\subsection{Implicit Input}

\subsection{Named Variables Only For Advanced Functionality}

\subsection{Building Programs Top Down}


From the above example, we have an understanding of how the system works.  The mental model that the user has when doing the task is to do the task that they want automated as they normally would while giving instructions to the computer about the decision point 


1. Do the program as the person normally does

2. specify the variables that you want the system to recognize

3. describe the control flow

4. specify the data you want the program to run on


Different interfaces seem better suited for different inputs and outputs. During initial prototypes we noticed that certain actions were more easy with certain input or output modalities.  For example, when inputting data into a program, it was easier to do with with mouse and keyboard than it was with voice.  However, when describing what the program should do, it felt more natural to describe using voice how the program should work than it was to do with mouse and keyboard.

Thus we separated different programming tasks to different modalities:

\subsection{Voice for Control Flow}
When testing the system, people said that they found the voice to be the easiest input modality over a graphical user interface.  We hypothesize that to non-programs, describing programming concepts with a GUI is daunting because they are not familiar with it.  A natural language interface though is easier to use and more user friendly.




==> survey.tex <==
\subsection{Survey on Interest in Skill Automation}

We had a wide range of users participating in the study.  In total we had 38 valid responses.   The most common group was were people that described themselves as managers.  The second most common group was people that worked in retail.

The gender of survey respondents was tilted towards men; this is likely explained due to the demographics of Mechanical Turk, which we used because of COVID-19. 66\% of respondents were male and 33\% of respondents were female.

There was a good distribution of programming skills. 25\% had never done any computer programming, 28\% had done light programming (Office macros and excel functions), 19\% were beginner programmer (around 1-2 college level computer science classes), 11\% were intermediate programmer (1-2 years of programming experience), and 17\% 1experienced programmer (2 or more years of programming experience).

Respondents were frequent users of virtual assistants. 64\% used a virtual assistant at least once a day, 30\% at least once a week, and 6\% said they used a virtual assistant less frequently than once a week.

\subsubsection{Desired Skills} \label{sec:user_study_results}
Of the skills that people wanted to do, 15\% of could be done Alexa (alarms, setting calendar appointments, buying products online), but 85\% were not possible on Alexa.  Skills that could not be done on Alexa because the an API  did not exist (``order food from a local restaurants''), there was not a GUI (``sorting values from a chart''),  or lack of conditions (``set an alarm if it is raining'').
98\% of the skills people wanted could be done in the web browser, although 2\% of skills people wanted to run on their local computer (``remove all the temporary files on my computer'').

Less than >1\% involved capabilities that our system was not able to handle for a home surveillance system that would capture images when there is motion.

The programming constructs that were needed to facilitate the skills that are doable by our system are as follows: 21\% trigger, 27\% iteration, 22\% no programming construct needed, 16\% filter, 6\% conditional, 3\% trigger and conditional, 2\% filter and conditional


==> system.tex <==
\section{System}
\label{sec:system}

WebAutomator is backed by a formal language we call \WebTalk. This language is an extension of the ThingTalk language~\cite{almondwww17}, a previously proposed programming language for voice assistants. In this section, we introduce the \WebTalk language, and describe how the language leverages Puppeeter to automate web tasks.

\subsection{Recording \& Replaying Web Interactions}
\label{sec:puppeteer}

Web Automator can record the user interaction with websites, and construct scripts that call the Puppeteer APIs. Puppeteer is a well-known mechanism for programmatically controlling websites.
Web Automator defines the following high-level primitives, built on top of the Puppeteer API:


With these primitives, a user can construct a program that buys a certain amount of Google stock, like this:

\begin{lstlisting}
@load(url="https://example.com/stockbroker");
@set_input(selector="input#search", text="goog");
@click(selector="button[type=submit]");

@set_input(selector="input#amount", text="100");
@click(selector="button[type=submit]");
\end{lstlisting}

The program would be constructed by navigating to the ``https://example.com/stockbroker'' page, entering ``goog'' in the search field, clicking the submit button, then entering ``100'' in the amount field and submitting again.

The same program can be wrapped into a procedure, as:
\begin{lstlisting}
procedure buy_stocks() {
  @load(url="https://example.com/stockbroker");
  @set_input(selector="input#search", text="goog");
  @click(selector="button[type=submit]");

  @set_input(selector="input#amount", text="100");
  @click(selector="button[type=submit]");
}
\end{lstlisting}

At a later time, the user can replay the recorded script with the command with ``run buy stocks'', referring to the ``buy\_stocks'' procedure name. When the user issues the command executing a procedure, a new Puppeteer session is started in the background, and the statements executed in sequence. 

\subsection{The \WebTalk programming language}

Puppeteer commands are recorded in the form of \WebTalk programs. \WebTalk is a statically-typed, imperative domain-specific language inspired by ThingTalk, and optimized for incremental multi-modal construction. The formal definition of \WebTalk is given in Figure~\ref{fig:webtalk-definition}. Here we describe the constructs in \WebTalk in detail.

\paragraph{Primitive Statements}
The most primitive statements in \WebTalk invoke a single Puppeteer API, such as Click or Load. They are executed sequentially in the order they are written. \textit{Action statements} execute a Puppeteer API without returning result, while \textit{query statements} return the result to the user (or to the caller in case of a nested procedure). Query statements have the form:
\begin{align*}
  \textit{api} \Rightarrow \texttt{notify}
\end{align*}

For example, the following program consists of an action statement that loads the ``example.com'' page, and then selects the ``\#data'' element and reads it aloud to the user:
\begin{lstlisting}
@load(url="https://example.com");
@select(selector="#data") => notify;
\end{lstlisting}

\paragraph{Procedures}
Multiple \WebTalk statements can be wrapped in \textit{procedures}, which then can be called by name in action statements. Procedures can have \textit{input parameters}, which can be used inside the body of the procedure, and bound to values when the procedure is called. For example, the ``buy stock'' procedure from Section~\ref{sec:puppeteer} can be made general to any company as follows:
\begin{lstlisting}
procedure buy_stocks(stock : String) {
  @load(url="https://example.com/stockbroker");
  @set_input(selector="input#search", text=stock);
  @click(selector="button[type=submit]");

  @set_input(selector="input#amount", text="100");
  @click(selector="button[type=submit]");
}
\end{lstlisting}
It can then be called as:
\begin{lstlisting}
buy_stocks(stock="goog");
buy_stocks(stock="aapl");
buy_stocks(stock="msft");
\end{lstlisting}
As in ThingTalk, parameters to procedures are passed by name, as that improves translation from natural language.

Procedures can also call other procedures, which is a form of \textit{function composition}. They cannot call themselves though, directly or indirectly (the name of the procedure is not hoisted and is not available inside the procedure body), which eliminates true recursion. Avoiding recursion ensures that \WebTalk is not Turing-complete, which is important for translation from natural language.

\paragraph{Returning results}
Procedures can also return results to the caller, using a query statement. For example, the following procedure reads a stock quote, and returns it to the caller.
\begin{lstlisting}
procedure stock_quote(stock : String) {
  @load(url="https://example.com/stocks");
  @set_input(selector="input#search",
             text=stock);
  @click(selector="button[type=submit]"); 

  @select(selector="#today") => notify;
}
\end{lstlisting}

At most one query statement can appear in the procedure, but the query statement need not be last: it can be followed by additional action statements, that do not affect the return value. This allows the procedure to perform ``clean up'' actions (such as logging out) before returning to the caller.

\paragraph{Assignment Statements}
\WebTalk supports calling the Puppeteer's Select API, and then assigning the result to a variable, as:
\begin{lstlisting}
let x := @select(selector="td.data");
\end{lstlisting}
This statement read the content of all table cells with the ``data'' class, and assigns the textual context to the variable ``x''. Because a Puppetter Select call returns a collection of elements, assignment statements always represent collections.

Similarly, an assignment statement can call a procedure, and store the result of the procedure in the variable. Continuing the previous example, this statement assigns the stock quote of Apple to the variable ``apple\_stock''.
\begin{lstlisting}
let apple_stock := stock_quote(stock="aapl");
\end{lstlisting}
In this case too, the assignment statement represents a collection of element, as the procedure value comes from a query statement that necessarily selected a collection of elements.
It is a type error to call a procedure that does not return a result inside an assignment statement.

\paragraph{Iteration \& Parameter Passing}
Elements selected by a Puppeteer Select call, or referenced by assignment statement, can be iterated and used to call an action, using a \textit{query-action statement}. For example, the following program selects all elements in the ``stocks'' table cells, and calls the ``buy\_stock'' procedure on all of them:
\begin{lstlisting}
let stocks := @select(selector="td.stock");
stocks => buy_stocks(stock=text);
\end{lstlisting}
In this example, the ``buy\_stocks'' is called repeatedly for each HTML element selected by Puppeeteer, and it passed the ``text'' field as the ``stock'' parameter.

\paragraph{Aggregation and Element-wise Compute}
\WebTalk supports all the query operations supported by ThingTalk~\cite{schema2qa}.  Once a set of number is selected in either a table or list, the \textit{sum},  \textit{count}, \textit{average}, \textit{max}, and \textit{min} can be computed and returned.

\paragraph{Query Operations}
\WebTalk supports all the query operations supported by ThingTalk~\cite{schema2qa}. These include \textit{filtering}, \textit{sorting}, and \textit{indexing}, which subsets the selected element based on a logical predicate.

For example, this program first selects all table cells with value greater than 100, then computes the average and reads it out loud to the user:
\begin{lstlisting}
let large_cells := @select(selector="td"), number >= 100;
aggregate avg of large_cells => notify;
\end{lstlisting}

Filtering can also be used to implement conditionals. For example, the following program buys Google stock only if the quote is less than \$1000:
\begin{lstlisting}
let apple_stock := stock_quote(stock="aapl");
apple_stock, number <= 1000 => buy_stock(stock="aapl");
\end{lstlisting}
Note that in this program, ``apple\_stock'' is a collection of one element, and after filtering it contains either 0 or 1 elements. The action is then called for each element of the filtered collection, so either 0 or 1 time, effectively implementing the conditional.

\paragraph{Timers}
Following ThingTalk, \WebTalk includes support for interval and calendar-based timers, which specify that a certain action or procedure call is to be executed repeatedly at a certain interval or a certain time. For example, the following statements will execute the ``buy\_stocks'' procedure repeatedly twice a week, and repeatedly every day at 10am respectively:
\begin{lstlisting}
timer(interval=1week, frequency=2) => buy_stocks(stock="goog");
attimer(time=new Time(10, 0)) => buy_stocks(stock="goog");
\end{lstlisting}

Unlike ThingTalk, \WebTalk does not support arbitrary monitoring of API or procedure calls. This is because it does not know the correct rate of monitoring, and cannot prove that a certain procedure will not be free of side-effects (such as locking the user out) if monitored at a rate that is too high.

\iffalse
 and the open API library Thingpedia, a large repository of APIs and their natural language representation. Each statement in \WebTalk invokes an API call from Thingpedia. \WebTalk includes two kind of statements: assignment statements bind the result of invoking a Thingpedia query to a variable name, and action statement execute a Thingpedia action based on available data. Action statements have the form:

\begin{align*}
  \textit{data}, [\textit{filter}]? \Rightarrow \textit{action}~\texttt{;}
\end{align*}

Which reads as “for every element of data, if the filter condition is satisfied, execute the action”. data refers to a variable in scope, and filter is a boolean expression that can use numeric and string comparison operators. action is a call to a Thingpedia action function.
For example, the following \WebTalk program reads the stock market results for Alphabet, then buys it if it is growing more than 10\%:

\begin{lstlisting}

let stocks := @stocks.get_quote(stock_id="goog");
stocks, increase_pct >= 10 => @stockbroker.buy(stock_id="goog", amount="$100");

\end{lstlisting}

In this example, the  \verb|stocks| variable is a list of named tuples, with fields \verb|increase_pct| and \verb|stock_id|. The fields are bound to automatic variable within each statement and can be used in the action for parameters of the same name.

\WebTalk statements can be grouped in procedures. Procedures are given a name by the user, and have formal parameters which are bound when the procedure is executed. For example, the previous stock program can be made independent of the company as follows:

\begin{lstlisting}

let procedure buy_if(p_stock_id : String) := {
    let stocks := @stocks.get_quote(stock_id=p_stock_id);
    stocks, increase_pct >= 10 => @stockbroker.buy(stock_id=o_stock_id, amount="$100");
};
\end{lstlisting}

At a later time, the user can invoke the procedure with a statement of the form:

\begin{lstlisting}
buy_if(p_stock_id="goog");
\end{lstlisting}
\fi

\iffalse
\subsection{Accessing Puppeeter from the \WebTalk language}
To access the data and control web pages, we extend Thingpedia with a new skill that binds the Puppeteer API. The skill includes the following operations:



Using the Puppeeter API, the previous stocks example can be constructed in terms of operating on web pages:

\begin{lstlisting}
 let procedure buy(p_stock_id : String) := {
    @load(url="https://example.com/stockbroker");
    @set_input(selector="input#search", text=p_stock_id);
    @click(selector="button[type=submit]");

    @set_input(selector="input#amount", text="100");
    @click(selector="button[type=submit]");
};
 let procedure buy_if(p_stock_id : String) := {
    @load(url="https://example.com/stocks");
    @set_input(selector="input#search", text=p_stock_id);
    @click(selector="button[type=submit]"); 

    let stock_increment := @select(selector="#today-increase");
    stock_increment, number >= 10 => buy(stock_id=p_stock_id);
};
\end{lstlisting}

The first procedure replaces the Thingpedia skill for the brokerage account, while the second procedure operates on a public stock quote website. The (fictional) CSS selectors refer to the elements on the page containing a search box (to navigate to the correct stock) and a form to buy stocks. The second procedure makes use of the first one to complete the buying transaction. This example shows that WebAutomator and Puppeteer can replace hand-coded voice assistant skills with skills that are custom-built by end-users.
\fi

\subsection{Multimodal Program Specification}
WebAutomator can construct complex WebAutoTalk programs, with multiple statements and recursive procedure calls. It does so one statement at a time. While recording, WebAutomator maps each action the user performs and each natural language sentence from the user into a WebAutoTalk statement. Statements are grouped into procedures explicitly by the user, who also chooses the name of the procedure.
WebAutomator records all the input of the user into editable elements, which is mapped to @SetInput calls. The user can also give a name to the input, in which case the input is bound to a fresh formal parameter of the current procedure. WebAutomator records also all clicks to active elements (links and buttons) and navigations between pages.
The user can also select parts of the page to use as data in subsequent statement. WebAutomator maps that operation to a @Select call, and binds the result to the name given by the user.
Finally, the user can call previously named procedures, as well as other skills defined in Thingpedia. When it does so, the user can refer to the data it has selected, by name. WebAutomator then binds the variables holding the selection in the current program to the actual parameters of the procedure call. 

For example, the ``buy\_stocks'' procedure in the running example can be constructed as follows:

\begin{itemize}
  \item User opens the \texttt{https://example.com/stockbroker} web page
  \item User says “begin recording”. WebAutomator records the Load operation in Puppeteer
  \item User types “goog” in the search box (with CSS selector “input\#search”) then says “this is a stock”. WebAutomator creates a “stock” formal parameter for the current procedure, then adds a SetInput operation
  \item User clicks the Search button. WebAutomator records a Click operation.
  \item User types “100” in the amount box (with CSS selector “input\#amount"). WebAutomator adds a SetInput operation. The user does not name this parameter, so it is recorded as a literal value.
  \item User clicks the “Buy” button. WebAutomator records a Click operation
  \item User says “name this program buy stocks”. WebAutomator now creates the ``buy\_stocks'' procedure, and remembers it for future usage.
\end{itemize}

\iffalse
Similarly, the second part of the stock example can be constructed as:

\begin{itemize}

  \item User opens the \url{https://example.com/stockquotes} web page
  \item User says “begin recording”. WebAutomator records the Load operation in Puppeteer
  \item User types “goog” in the search box (with CSS selector “input\#search”) then says “this is a stock id”. WebAutomator creates a “p\_stock\_id” formal parameter for the current procedure, then adds a SetInput operation
  \item User clicks the Search button. WebAutomator records a Click operation.
  \item User selects the percent increase for today on the web page (with CSS selector ``\#today-increase'') and says “This is a stock increment”. WebAutomator adds a call to the Puppeteer Select API and then records the result in the stock\_increment variable.
  \item User says “call buy with stock id if stock increment is greater than 10”. WebAutomator adds the statement that calls the buy procedure. It makes use of the “stock\_id” variable, which is bound to the stock\_id formal procedure parameter. The action is conditional on the stock increment, bound to the selection on the page.
\end{itemize}
\fi

\iffalse
\subsection{Constructs}

Our system supports four different constructs of procedure execution: (1) for each, (2) if, (3) trigger, and (4) filter.

\subsubsection{Iteration}
After declaring a procedure with a variable in recording mode, the user can select a list of items and assign them a single variable name. The user can then call the procedure with this list of items, causing the actions in the procedure to be reenacted for each of the items in the selected list.

\subsubsection{Conditional}
A user can request a procedure be executed if a previously defined numerical element on the page is less/greater than or equal to a certain value.  

\subsubsection{Trigger}
A procedure can be scheduled for a certain time in the day, at which it is executed. The time uttered by the user is passed to a natural language understanding engine developed by the Stanford Open Virtual Assistant Laboratory, which can parse the time from a variety of different formats.

\subsubsection{Filter}
The user can ask our system to highlight certain elements on a page that match a certain condition. For example, the user can ask for items in a selected and named table of restaurants for those with reviews greater than three and a half stars. Items highlighted are moved to the top of the page to be easily visible in the user’s field of view. 

\subsubsection{Compounds}
TODO
\fi


==> user_primitives.tex <==
\section{User Primitives}
Once a user says a command it is translated from speech into text.  This utterance is then matched to a primitive action.  For each primitive action, their are a number of similar paraphrases that the user can also say which map to the same primitive.   Paraphrases were developed  by observing through an iterative process of user feedback to determine which utterances people naturally gravitated towards.

\subsection{Natural Language}


\subsubsection{Conditionals}
As the user is building the program, they can use their voice to specify conditions on which the program should run. A program can be set to run if a variable that the user has created is less than or greater than a specified value. 


Example paraphrases: 
``call \texttt{:prog\_name} if \texttt{:var\_name} is at least \texttt{:value}''

% ``call \texttt{:prog\_name} if \texttt{:var\_name} more than \texttt{:value}'',
% ``call \texttt{:prog\_name} if \texttt{:var\_name} is greater than \texttt{:value}'',
% ``call \texttt{:prog\_name} if \texttt{:var\_name} equals \texttt{:value}'',
% ``call \texttt{:prog\_name} if \texttt{:var\_name} is at most \texttt{:value}'',
% ``call \texttt{:prog\_name} if \texttt{:var\_name} is less than \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} more than \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} is greater than \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} is at least \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} equals \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} is at most \texttt{:value}'',
% ``run \texttt{:prog\_name} if \texttt{:var\_name} is less than \texttt{:value}''





\subsection{Outputs}

\subsubsection{Audio}
The system uses audio to speak to the user.  After a user has complete an action, the system will prompt  the user on a suggested next step.

The actions that a user can take with a traditional user interface are discoverable through buttons and menus.  If a task requires a series of actions, software like a wizard is used to lead a user through a series of steps.  The benefit of this is that the user always knows what action to do next.  With a natural language interface, users can be left uncertain what is their next step.  We break this down into two components.  The first is what is the action that they should take next and the second is how they should describe the action.


\subsubsection{Text}
Values returned from a program are often in list form and can be long.  When results are returned a pop-up window of the values are shown to the user.  The user can then use these values as input into another program.  The popup is done out of band so the results can be piped to another program.

